A Practical Approach to Combinatorial Test Design

Typical software has a huge input space. The number of inputs may be astronomical or even infinite. Thus, the task of validating that the software is correct seems hopeless. To deal with this difficult task, Combinatorial Test Design (CTD) can be used to provide reduction of the testing space and high quality and efficient testing. The application of CTD is largely determined by the quality of the CTD model. This book covers the CTD test design methodology and CTD modeling in details. It elaborates on the process of constraints definition. It also explains how to best define your coverage requirements to direct and focus your tests. It is hard to create good CTD models without a good grasp of the implementation of CTD tooling. To that hand, the book also takes a deeper dive into covering principles and algorithms needed to build CTD tooling. Hands on exercises are used throughout the text and help create a clear understanding of the concepts covered within this book.

==> introduction.tex <==
\chapter{Introduction}

The last decade has seen unprecedented growth in the deployment of Machine Learning (ML) based solutions, %(sometimes referred to as AI),
broadly influencing many aspects of our lives \cite{CNN2019}. %\footnote{See CNN 2019 article for more details -  \href{https://edition.cnn.com/2019/12/21/tech/artificial-intelligence-decade/index.html}{https://edition.cnn.com/2019/12/21/tech/artificial-intelligence-decade/index.html}} 
Significant progress has been made in machine learning tasks such as image recognition, language translation, and tasks related to self-driving cars, to name a few. With such prospects of potential success, the industry is attempting to apply ML to a variety of use cases at an unprecedented rate, including crime prevention, medicine, IT and cloud analysis, cyberspace security, intelligent chatbots, and many more. %various "AI agents" that provide services in various domains.  


ML-based systems combine ML models and regular software to achieve some common goal, e.g., making the driving decisions of the self-driving car. But what are ML models? ML models can be thought of as regular computer programs that were produced by automatically searching over some predefined set of possible programs.  The search is guided by examples of the desired program behavior.  We usually refer to the examples as the training data or simply as data.  Thus, just as we teach young children by example, in the case of ML models, we provide the machine with examples from which it learns the correct behavior; hence, the name machine learning.    


ML models are statistical by design. We do not expect to find an ML model that is always correct.  In fact, we are unlikely to know whether the space of possible models that we search in contains such a perfect model, and even if it does it may be too difficult to find.  Instead, we settle for the model being correct most of the time.  In addition, we require that a successful model will be correct most of the time on unseen data of the same type as the data it was trained on.  %We call this desired trait generalization.  
This trait is commonly referred to as {\em model generalization}. Thus, a bug in an ML model usually cannot be determined from the individual response of the model to a single data point; rather, it is determined by the aggregated behavior of the ML model on many examples. As a result, an ML solution composed of several ML models and regular software can only be successfully crafted if it is validated by statistical experiments.   It also means that the required behavior of an ML solution can only be defined as an aggregate of its behavior on individual data points. Therefore, the control of the aggregated statistical behaviour of the crafted ML system as a whole is indeed a major challenge addressed in this book. The average aggregate behavior and its control can be exemplified in the case of a self-driving car. For example, we can specify that the desired average number of wrongly recognized type of vehicle is no more than 5\%.

With this in mind, we emphasize the need for well-defined quantitative measures that reflect the desired behavior of the ML-based system. An example of such a measure is the average number of service calls a chatbot, whose goal is to address those calls autonomously, is routing to a human service agent. Such measures can be derived from {\em statistical functional requirements} hence denoted {\em statistical functional measures} or SF measures in short. Once SF measures are properly defined, one can utilize them to analyze the desired behavior of the system. As described in this book, this analysis can be performed via appropriately designed statistical experiments that estimate the expected average and variance of the SF measures. A good experiment should provide accurate estimates of the SF measures when the ML-based system is deployed. This practice of defining SF measures and designing experiments that test them throughout the life-cycle of the ML-based system tackles the challenge of crafting an ML-based system that meets its requirements. 

Collecting a set of training examples for a given SF requirement is challenging too. The data may be lacking factors without which the desired model cannot make correct decisions. We might have too few examples, or examples that are not representative of the type and distribution of data that the system will encounter when deployed. %the model is applied.
Finally, in order to guide the learning, the data needs to include the "correct answer" as well as indication that it is indeed correct. Such indication is typically provided %refer to that as
by labeled data, in which case the problem is a supervised learning problem. However, it often happens that an organization holds a representative set of examples that is readily available but are not labeled.  

As suggested above, this book aims to address the challenges of crafting robust ML solutions that meet their design requirements and in particular SF requirements, and hence can be confidently deployed. We focus on an experimental approach to the crafting of ML solutions. This approach can be thought of as the ML equivalent of the test-first approach applied to regular software. To emphasize this similarity, we name our approach {\em experiment-first}. The focus of this approach is on crafting, validating, and continually monitoring ML-based solutions via a series of carefully designed experiments at different levels of abstraction. The book is self-contained and addresses the mathematical and statistical techniques needed to apply the experiment-first approach.  It contains numerous practical programming as well as theoretical exercises and their solutions. Exercises are an integral part of the text and are designed to facilitate understanding of the ideas, concepts and methods introduced. 

The main target audience of this book is data scientists who craft ML-based solutions, architects who define what the solutions need to do, and testers who need to validate that the system actually works and meets its specifications. The book also attempts to bridge communication gaps between the stakeholders involved in the development of ML-based solutions. The experiment-first approach introduced in this book facilitates an end-to-end, unambiguous, quantitative definition of the steps to be taken in the development of an ML-based system. Our approach details the activities performed, and the artifacts consumed and generated, throughout the development and deployment of the solution. 
The book introduces the statistical experiment and its results as the language by which the stakeholders communicate effectively to craft the ML-based solution.        

A preferred way to design and implement experiments entails following a scientific experimental methodology. This methodology includes the definition of a problem, the formulation of a quantitative conjecture, and the design and implementation of an experiment that validates or rejects the conjecture.  For example, a problem could consist of finding the speed at which a ball will touch the ground when dropped from a high tower.  The conjecture is that the speed is proportional to the time, and the experiment involves dropping balls from towers of different heights and measuring how long it takes them to hit the ground. 

This book is organized as follows. In Chapter \ref{Chapter:scientific-method} we paint in broad strokes the scientific experimental methodology and highlight its applicability %relation 
to ML system development and validation. As mentioned in the previous paragraph, following the scientific methodology includes defining a problem, making a conjecture about how the problem may be solved, and then designing and implementing an experiment to validate the conjecture.  When crafting an ML-based solution, the standard conjecture entails generalization, namely, that the system will behave as required on new inputs not seen before.  The problem that the conjecture implicitly aims to solve is being able to construct an ML-based system that meet the requirements on new data.  After defining the requirements we address specifics of how to formulate a generalization conjecture and how to craft the appropriate experiment to validate it and analyze the results in the event that the conjecture was wrong. We also discuss %highlight 
the way in which the results of the experiments influence system design and contribute to the continual monitoring and validation of the system throughout its life-cycle.  

Then, Chapter \ref{mindDirect} details practical aspects of the experiment-first methodology. They are described as a set of best practices and pitfalls that aim to quickly reduce the risks associated with the development of the ML-based system and help address the most important concerns first.  Practices proposed in Chapter \ref{mindDirect} should allow stakeholders to better validate, from day one, the potential for successful generalization given the business requirements and data. The practices should additionally identify optimal usage of information extracted from the data and application of the most suitable ML techniques to the problem at hand. % It is highly beneficial to repeatedly come back to these practices with teams as they are applied in practice.  

When analyzing ML models, the focus is sometimes on generic performance measures, e.g., the accuracy of the model. In contrast, an ML-based solution has unique, specific SF requirements. For example, a service chatbot may be required to autonomously handle at least $90\%$ of its conversations with customers, and send at most $10\%$ of to a human service agent for processing. In addition, specific requirements are frequently realized through the interaction among ML models and regular software.  Chapter \ref{unitSystem} discusses the composition of ML software and regular software in a unified ML-based system, and how such composition impacts system validation.


The next two chapters on ML testing before deployment (Chapter \ref{Chapter:MLtesting}) and on drift (Chapter \ref{Chapter:drift}) address the system correctness concern at different phases of the system life cycle. The ML testing chapter focuses on checking system correctness before it is deployed, while the chapter on drift detection analyzes whether the system operates correctly once it is deployed.  

%As the basic 
Generalization is a fundamental conjecture made about ML-based system correctness. % entails the generalization of some measure, e.g., the volume of service calls that were sent to a human agent in a chatbot scenario, 
Thus, the experiments performed at testing time should indicate %project 
that the desired behavior will manifest once the system is deployed. Due to the stochastic nature of ML-based systems, the validation typically includes a stability assertion %claim.  A claim 
An assertion could suggest, e.g., that on average, 5$\%$ of the service calls received by a service chatbot are diverted to a human service agent, but it is unlikely that more than 10$\%$ of the calls are diverted. 
As data changes over time the system might fail to meet the desired behavior once it is in operation, even if it was well built and tested. For example, in the chatbot scenario, changes in the type of service calls might result in much more than 10$\%$ of the calls being diverted to a human agent. To handle this, drift detection is required. This topic is addressed in Chapter \ref{Chapter:drift}.  

Once the expected system behavior is established, we can define an optimal business process. % that is based on the system expected behaviour.  
In the chatbot example, once we know that up to 10$\%$ of the service calls are diverted to a human agent, we can plan the size of the customer service team that will provide proper response to the diverted calls. The integration of ML-based system behavior with the business process is discussed in Chapter \ref{optimal}. Finally, 
%
in Chapter \ref{industrial}, we present an industrial example to demonstrate the implementation of principles of the experiment-first methodology in practice.
%
Solutions to exercises that appear across the book. Code samples and mathematical background are found in the appendix. 

This concludes the description of the content of this book. It is important to note that the book does not cover topics such as generic trust-related measures and MLops. %We elaborate on this below.  
%
ML models learn from data. Hence, their inferences may be affected by data bias and adversarial manipulation. %For example, gender bias in the ML model may result when learning from historical data. In addition, data can be manipulated by attackers to change the learning results. 
Some ML models can be trusted only if their decisions are comprehensible. %This concern is especially prominent in the legal context. For instance, a court of justice may require an explanation of the rationale behind a decision made by the ML model.
Much research addresses these concerns \cite{trust}, \cite{RSG2016}.
%
%The above concerns are sometimes collectively referred to as trust concerns. This book does not focus on trust concerns. %directly. Instead, when following the experiment-first methodology, the appropriate set of trust concerns that are relevant to the ML solution at hand will naturally surface as the system requirements are defined. This will then lead to the design of experiments that address these trust concerns. 
%At that point, it is advisable to apply state-of-the- art techniques related to trust and model readability\cite{10.1145/2939672.2939778}. 
%
%The book additionally does not address %
Low-level engineering concerns (e.g., automatic model re-training) are out of scope too, %, saving the data that was used for training, and tracing it to the model that was obtained from the training. These topics are well covered in the literature (see, 
and are well covered in the art (e.g., MLops tutorial \cite{MLops}). 
% \href{https://towardsdatascience.com/get-started-with-mlops-fd7062cab018}{\underline{see tutorial on MLops.}}. XX-Onn


  
  

==> numpy.tex <==
\noindent The actual data in the dataframe is actually an \textit{ndarray} in NumPy (A multidimensional homogeneous array). That means we can do operations on the data using NumPy. For example, if you have a dataframe \textit{df1}, the \textit{ndarray} would be extracted by doing

\begin{lstlisting}[style=python]
nd1 = df1.values
\end{lstlisting}

\noindent Accessing a cell in the array is as simple as:

\begin{lstlisting}[style=python]
val = nd1[row,col]
\end{lstlisting}

\noindent You can also access subarrays by indexing with the colon:

\begin{lstlisting}[style=python]
sub = nd1[0:3,1:3]
\end{lstlisting}

\noindent would capture the rectangular subarray from the first to the third rows and the second to third columns.

\paragraph{Indexing} Note that the second part of the index is 1 past the actual index that will be the last, so 0:3 only pulls out 0,1, and 2.

\noindent Like in MATLAB, you can pull out everything using just the colon. For example:

\begin{lstlisting}[style=python]
sub = nd1[3,:]
\end{lstlisting}

\noindent would retrieve all columns of row 3.

\paragraph{Negative indexing} To get the last index, you can use negative numbers (the last index would be -1, second to last -2, etc.)

\begin{lstlisting}[style=python]
sub = nd1[-1,1:3]
\end{lstlisting}

\noindent would get columns 1,2 of the last row.

\paragraph{Boolean indexing/masking} Suppose we want to get the values in an array, $a$, which are all less than the mean. NumPy's masking feature makes it really intuitive, as all you need to do is:

\begin{lstlisting}[style=python]
lessThanMean = a[a<a.mean()]
\end{lstlisting}

\noindent The array $a < a.mean()$ would be a boolean array, which might look like
\begin{lstlisting}[style=python]
[[True, True, False, False]]
\end{lstlisting}

\paragraph{Assignment} Assigning values in an array is easy using the NumPy notation. For example, say we wanted to replace the values in the first 2x2 square of \textit{nd1} with the 2x2 square in nd2 with columns 2 and 3, and rows 3, and 4. The operation would be:

\begin{lstlisting}[style=python]
nd1[0:2,0:2] = nd2[-2:,2:4]
\end{lstlisting}

\paragraph{Creating an array} Creating a numpy array is as easy as passing in a normal python list into the array method:

\begin{lstlisting}[style=python]
import numpy as np

print np.array([1,2,3])
\end{lstlisting}

\noindent Creating a 2D $mxn$ array is as simple as passing in a $m$-long list of $n$-tuples.

\begin{lstlisting}[style=python]
import numpy as np

print np.array([(1,2,3),(4,5,6)])
\end{lstlisting}

\noindent would output

\begin{lstlisting}[style=python]
[[1,2,3]
 [4,5,6]]
\end{lstlisting}

\paragraph{More initializers} You can also create arrays with certain initial values.

\begin{lstlisting}[style=python]
np.empty((5,3,2))
\end{lstlisting}

\noindent initializes an "empty" $5x3x2$ dimensional array. The values in the array are actually whatever was in the memory locations of the array pointers, so the output could look like garbage.

\begin{lstlisting}[style=python]
np.ones((5,4), dtype=np.int)
\end{lstlisting}

\noindent creates a $5x4$ array, where the value in each cell is the integer 1.

\begin{lstlisting}[style=python]
np.random.random((5,4))
\end{lstlisting}

\noindent creates a $5x4$ array with random numbers from a uniform distribution in [0.0,1.0). An example result could be:

\begin{lstlisting}[style=python]
[[ 0.82897637  0.36449978  0.91209931  0.96307279]
 [ 0.63777312  0.24482194  0.5817991   0.18043012]
 [ 0.85871221  0.98874123  0.68491831  0.53831711]
 [ 0.52908238  0.81083147  0.97440602  0.81032768]
 [ 0.98566222  0.38902445  0.16922005  0.0873198 ]]
\end{lstlisting}

\noindent Other methods or fields, such as $sum()$ or $size$ can be looked up in online documentation.
